On Reinforcement Learning for Turn-based Zero-sum Markov Games

We consider the problem of finding Nash equilibrium for two-player turn-based zero-sum games. Inspired by the AlphaGo Zero (AGZ) algorithm, we develop a Reinforcement Learning based approach. Specifically, we propose Explore-Improve-Supervise (EIS) method that combines "exploration", "policy improvement"' and "supervised learning" to find the value function and policy associated with Nash equilibrium. We identify sufficient conditions for convergence and correctness for such an approach. For a concrete instance of EIS where random policy is used for "exploration", Monte-Carlo Tree Search is used for "policy improvement" and Nearest Neighbors is used for "supervised learning", we establish that this method finds an $\varepsilon$-approximate value function of Nash equilibrium in $\widetilde{O}(\varepsilon^{-(d+4)})$ steps when the underlying state-space of the game is continuous and $d$-dimensional. This is nearly optimal as we establish a lower bound of $\widetilde{\Omega}(\varepsilon^{-(d+2)})$ for any policy.

==> ais_tex_files/app_Boltzmann.tex <==
\section{Proof of Proposition~\ref{prop:Boltzmann}} \label{appendix_proof_Boltzmann}

\begin{proof} Let $N=N_h.$ 
We first show that the expected time to obtain a
$(h,1)$-representative set under Boltzmann policy is upper bounded by 
$T(h,1)=O\left(\frac{n\left|\mA\right|}{\alpha\varphi\nu_{\min}}\log N \right).$ Note that if all the balls
$\{B_{i},i\in[N]\}$ with radius $\frac{h}{2}$ are visited at least once, the set of sampled states will be $(h,1)$-representative. Without loss of generality, we may assume that the balls are disjoint, since the covering time will only become smaller if they overlap with each other. 

Recall that the Boltzmann policy $\hat{\pi}$ is based on the Q-value estimates $\hat{Q}(s,a)$, which is obtained from the MCTS module. Note that $\hat{Q}(s,a)\in[-V_{\max},V_{\max}].$ For each $s\in \mS_1,$ $a\in\mA$,we have
\begin{align*}
    \hat{\pi}(a|s)=\frac{\exp\left(\hat{Q}(s,a)/\tau\right)}{\sum_{a'}\exp\left(\hat{Q}(s,a)/\tau\right)}
\ge\frac{\exp\left(-V_{\max}/\tau\right)}{\left|\mathcal{A}\right|\exp\left(V_{\max}/\tau\right)}=:\alpha.
\end{align*}
Similarly, for each $s\in \mS_2,$ $a\in \mA,$ 
\begin{align*}
    \hat{\pi}(a|s)=\frac{\exp\left(-\hat{Q}(s,a)/\tau\right)}{\sum_{a'}\exp\left(-\hat{Q}(s,a)/\tau\right)}\geq \alpha.
\end{align*}

Hence for all $t\geq0,$ for all $s\in S,$ we have 
\[
\P_{\hat{\pi}}\big(a_{t}=\hat{a}_{1},\ldots,a_{t+n-1}=\hat{a}_{n}|s_{t}=s\big)\geq\big(\frac{\alpha}{|\mathcal{A}|}\big)^{n}.
\]

The equation~(\ref{eq:unif.erg.single}) implies that 
\begin{align}
	&\P_\pi\left(s_{t+n}\in \cdot |s_t=s\right) \nonumber \\
	\geq & \P\left(s_{t+n}\in \cdot |s_t=s, a_t=\hat{a}_1,\ldots,a_{t+n-1}=\hat{a}_n\right) \times \P_{\hat{\pi}}
	\left(a_t=\hat{a}_1,\ldots,a_{t+n-1}=\hat{a}_n|s_{t}=s\right)\nonumber \\
	\geq& \psi \nu(\cdot) \left(\frac{\alpha}{|\mA|}\right)^n. \label{eq:ergodic_eps}
\end{align}

First assume that the above assumption holds with $n=1$. Let $(\mathcal{P}_{1},\ldots,\mathcal{P}_{N})$ 
be a fixed ordering of the balls $\{B_{i},i\in[N]\}$. For each integer $t\ge1$,
let $W_{t}$ be the number of ball-action pairs visited up to time
$t$. Let $T\triangleq\inf\left\{ t\ge1:W_{t}=N\right\} $ be the
first time when all balls are visited. For each $w\in\{1,2,\ldots,N\}$,
let $T_{w}\triangleq\left\{ t\ge1:W_{t}=w\right\} $ be the the first
time when the $w$-th ball is visited, and let $D_{w}\triangleq T_{w}-T_{w-1}$
be the time to visit the $w$ ball after $w-1$ balls have been
visited.  We use the convention that $T_{0}=D_{0}=0$. By definition,
we have $T=\sum_{w=1}^{N}D_{w}.$ 

When $w-1$ pairs have been visited, the probability of visiting a \emph{new} ball is at least 
\begin{align*}
	&\min_{I\subseteq[N],\left|I\right|=N-w+1}\P\Big\{ s_{T_{w-1}+1}\in\bigcup_{i\in I}\mathcal{P}_{i}|s_{T_{w-1}}\Big\}  \\
	=& \min_{I\subseteq[N],\left|I\right|=N-w+1}\sum_{i\in I}\P\left\{ s_{T_{w-1}+1} \in\mathcal{P}_{i}|s_{T_{w-1}}\right\} \\
	\ge& (N-w+1)\min_{i\in[N]} \P \left\{ s_{T_{w-1}+1} \in\mathcal{P}_{i}|s_{T_{w-1}}\right\} \\
	\ge& (N-w+1)\cdot\varphi\nu_{\min}\cdot\frac{\alpha}{|\mA|},
\end{align*}
where the last inequality follows from Eq.~(\ref{eq:ergodic_eps}).
Therefore, the time to visit the $w$-th pair after $w-1$ pairs have been visited, $D_{w},$ is stochastically dominated by a geometric random
variable with mean at most $\frac{\left|\mA\right|/\alpha}{(N-w+1)\varphi\nu_{\min}}.$
It follows that 
\begin{align*}
	\E T & =\sum_{w=1}^{N}\E D_{w}\le\sum_{w=1}^{N}\frac{\left|\mA\right|/\alpha}{(N-w+1)\varphi\nu_{\min}} =O\left(\frac{\left|\mA\right|/\alpha}{\varphi\nu_{\min}}\log N\right).
\end{align*}
This prove that the expected time to sample a $(h,1)$-representative set is upper bounded by $T(h,1)=O\left(\frac{\left|\mA\right|/\alpha}{\varphi\nu_{\min}}\log N\right)$ for $n=1$. For general values of $n$, following from a similar argument
by considering the Markov game only at times $t=n,2n,3n,\ldots,$ we have
\begin{align*}
    T(h,1)=O\left(\frac{\left|\mA\right|^n}{\alpha^n\varphi\nu_{\min}}\log N\right).
\end{align*}

Note that if the trajectory samples $K$ $(h,1)$-representative sets, then each state in the space has at least $K$ neighbors within distance $h$ in the set of observed states. Therefore, $KT(h,1)$ gives an upper bound for the expected time to visit a $(h,K)$-representative set starting from any state $s\in \mS.$ That is, 
\begin{align*}
    T(h,K)=O\left(\frac{K\left|\mA\right|^n}{\alpha^n\varphi\nu_{\min}}\log N\right).
\end{align*}

\end{proof}


==> ais_tex_files/app_instance.tex <==
\section{Proof of the Main Result: Theorem~\ref{thm:Approxiate_AGZ}}
 This section is devoted to the proof of Theorem~\ref{thm:Approxiate_AGZ}. We start with analyzing the MCTS oracle, drawing inspiration from the non-asymptotic analysis of MCTS for MDPs in~\cite{shah2019mcts}. We then show how the combination of MCTS's improvement property and the generalization of supervised learning iteratively refines the estimation model $f_{\theta_L}.$



\subsection{Proof of Theorem~\ref{thm:Approxiate_AGZ}} \label{subsec:approx_agz_proof}

To prove Theorem~\ref{thm:Approxiate_AGZ}, we start with the following lemma that characterizes the KL divergence of two Boltzmann policies.

\begin{proof} ({\bf Theorem~\ref{thm:Approxiate_AGZ}}) We first introduce some notion. For the $l$-th iteration (line 2): the depth
used in the MCTS oracle is given by $H^{(l)}$, and let the number of simulations
for each fixed depth MCTS query be $m_{l}$. The output of MCTS oracle
for the query state $s\in S$ is given by $\{\hat{V}(s),\{\hat{Q}(s,a)\}_{a\in \mA}\},$
Let $\hat{\pi}(\cdot|s)$ be the Boltzmann policy with respect to
the estimated Q-values $\{\hat{Q}(s,a)\}_{a\in \mA}$ using temperature
parameter $\tau_l$. We use $\mathcal{D}^{(l)}=\Big\{\big(s_{i},I(s_i),\hat{V}(s_{i}),\hat{\pi}(\cdot|s_{i})\big)\Big\}_{i=1}^{n_l}$
to denote the set of data generated by the MCTS oracle, and let $S^{(l)}=\{s_{i}\}_{i=0}^{n_{l}}$
be the set of states sampled. We denote by $Z^{(l)}$ all the information
during the $l$-th iteration, i.e., all the data observed in the MCTS
oracle for obtaining training data $\mathcal{D}^{(l)}$. Let $\{\mathcal{F}^{(l)}\}$
be the sigma-algebra generated by the stochastic process $\{Z^{(l)}\}.$
The error bounds for the value function and policy derived from the MCTS oracle are denoted by $\varepsilon_{v}^{(l)}$
and $\varepsilon_{p}^{(l)}$, respectively: 
\begin{align*}
\varepsilon_{v}^{(l)} & =\sup_{s\in S^{(l)}}\E|\hat{V}^{(l)}(s)-V^{*}(s)|,\\
\varepsilon_{p}^{(l)} & =\sup_{s\in S^{(l)}}\E\Big[D_{KL}\big(\hat{\pi}(\cdot|s)\Vert P_{l}^{*}(\cdot|s)\big)\Big],
\end{align*}
where $P_{l}^{*}(\cdot|s)$ is the Boltzmann policy with
respect to the optimal Q-function $\{Q^{*}(s,a)\}_{a\in \mA}$ using
temperature $\tau_l$. 

At the $l$-th iteration, supervised learning step takes the output
of the MCTS oracle, $\mathcal{D}^{(l)}$, as the training data. Let $\xi_{v}^{(l)}$
and $\xi_{p}^{(l)}$ denote the error bounds for the learned value function
$V_{\theta_{l}}$ and policy $P_{\theta_{l}}$, respectively. That is,
\begin{align*}
\xi_{v}^{(l)} & =\E\Big[\big\Vert V_{\theta_{l}}-V^{*}\big\Vert_{\infty}\Big],\\
\xi_{p}^{(l)} & =\sup_{s\in S}\E\Big[D_{KL}\big(P_{\theta_{l}}(\cdot|s)\Vert P_{l}^{*}(\cdot|s)\big)\Big].
\end{align*}
According to the generalization assumption on the supervised learning
oracle (cf. Property~\ref{property:sl}), when the size of training set $n_l$
is sufficiently large and the sampled states $S^{(l)}=\{s_{i}\}_{i=0}^{n_l}$
are representative  of the state space, the following
bounds hold
\begin{align*}
\xi_{v}^{(l)} & \leq c_{v}(n_l)\max_{i\in[m]}\E\big|\big[\hat{V}(s_{i})\big]-V^{{*}}(s_{i})\big|,\\
\xi_{p}^{(l)} & \leq c_{p}(n_l)\max_{i\in[m]}\E\Big[D_{KL}\big(\hat{\pi}(\cdot|s_{i})\Vert P_{l}^{*}(\cdot|s_{i})\big)\Big].
\end{align*}
Hence 
\begin{align}
\xi_{v}^{(l)} & \leq c_{v}(n_l)\varepsilon_{v}^{(l)},\label{eq:V_SL_bound_by_MCTS}\\
\xi_{p}^{(l)} & \leq c_{p}(n_l)\varepsilon_{p}^{(l)}.\label{eq:P_SL_bound_by_MCTS}
\end{align}

At the $(l+1)$-th iteration, the value function estimator $V_{\theta_{l}}(\cdot)$
obtained from the supervised learning oracle of $l$-th iteration
is used as the leaf node value estimator for the MCTS oracle. The property of MCTS (cf. Theorem~\ref{thm:mcts_game}) implies that for each query state~$s$,
the estimated V function $\hat{V}(s)$ and Q-values $\{\hat{Q}(s,a)\}_{a\in \mA}$
satisfy the following:
\begin{align*}
\E\Big[\big|\hat{V}(s)-V^{*}(s)\big|\ |\mathcal{F}^{(l)}\Big] & \leq |\mA|\gamma^{H^{(l+1)}}\omega_{v}^{(l)}+O\big(m_{l+1}^{\eta-1}\big),\\
\E\Big[\big|\hat{Q}(s,a)-Q^{*}(s,a)\big|\ |\mathcal{F}^{(l)}\Big] & \leq\gamma^{H^{(l+1)}}\omega_{v}^{(l)}+O\big(m_{l+1}^{\eta-1}\big),\quad a\in \mA
\end{align*}
where $\eta\in[1/2,1)$ is a constant, and 
\[
\omega_{v}^{(l)}\triangleq\big\Vert V_{\theta_{l}}-V^{*}\big\Vert_{\infty}.
\]
Note that $\xi_{v}^{(l)}=\E[\omega_{v}^{(l)}]$. Thus 
\begin{align*}
\E\Big[\big|\hat{V}(s)-V^{*}(s)\big|\Big] & \leq |\mA|\gamma^{H^{(l+1)}}\xi_{v}^{(l)}+O\big(m_{l+1}^{\eta-1}\big),\\
\E\Big[\big|\hat{Q}(s,a)-Q^{*}(s,a)\big|\Big] & \leq\gamma^{H^{(l+1)}}\xi_{v}^{(l)}+O\big(m_{l+1}^{\eta-1}\big).
\end{align*} 
Following Lemma~\ref{lem:KL}, we have
\begin{align*}
\E\Big[D_{KL}\big(\hat{\pi}(\cdot|s)\Vert P_{l+1}^{*}(\cdot|s)\big)\Big] %&\leq\frac{2}{\tau^{(l+1)}}\max_{a\in \mA}\Big\{\E\Big[\big|\hat{Q}(s,a)-Q^{*}(s,a)\big|\Big]\Big\}\\
 & \leq\frac{2|\mA|}{\tau_{l+1}}\Big[\gamma^{H^{(l+1)}}\xi_{v}^{(l)}+O\big(m_{l+1}^{\eta-1}\big)\Big].
\end{align*}
Therefore, we obtain that
\begin{align*}
\varepsilon_{v}^{(l+1)} & \leq |\mA|\gamma^{H^{(l+1)}}\xi_{v}^{(l)}+O\big(m_{l+1}^{\eta-1}\big),\\
\varepsilon_{p}^{(l+1)} & \leq\frac{2|\mA|}{\tau_{l+1}}\Big[\gamma^{H^{(l+1)}}\xi_{v}^{(l)}+O\big(m_{l+1}^{\eta-1}\big)\Big].
\end{align*}
Combining the above inequalities with Eqs. (\ref{eq:V_SL_bound_by_MCTS})\textendash (\ref{eq:P_SL_bound_by_MCTS})
yields
\begin{align}
\xi_{v}^{(l+1)} & \leq c_{v}(n_{l+1})\varepsilon_{v}^{(l+1)}\leq c_{v}(n_{l+1})\Big[|\mA|\gamma^{H^{(l+1)}}\xi_{v}^{(l)}+O\big(m_{l+1}^{\eta-1}\big)\Big],\label{eq:value_error_bound} \\
\xi_{p}^{(l+1)} & \leq c_{p}(n_{l+1})\varepsilon_{p}^{(l+1)}\leq\frac{2c_{p}(n_{l+1})}{\tau_{l+1}}\Big[|\mA|\gamma^{H^{(l+1)}}\xi_{v}^{(l)}+O\big(m_{l+1}^{\eta-1}\big)\Big]. \label{eq:policy_error_bound}
\end{align}
In particular, we have
\begin{align}
\xi_{v}^{(l+1)} &\leq \max \Big\{c_{v}(n_{l+1}),\frac{2c_{p}(n_{l+1})}{\tau_{l+1}}\Big\}\Big[|\mA|\gamma^{H^{(l+1)}}\xi_{v}^{(l)}+O\big(m_{l+1}^{\eta-1}\big)\Big],\nonumber \\
\xi_{p}^{(l+1)} &\leq \max \Big\{c_{v}(n_{l+1}),\frac{2c_{p}(n_{l+1})}{\tau_{l+1}}\Big\}\Big[|\mA|\gamma^{H^{(l+1)}}\xi_{v}^{(l)}+O\big(m_{l+1}^{\eta-1}\big)\Big]. \nonumber
\end{align}

Note that by Property \ref{property:sl}, $c_v(n)=O(1),$ and $c_p(n)=O(1)$.  Hence, for a given $\rho \in (0,1),$ we can choose the algorithm parameters in an appropriately way, in particular, the depth $H$ and the simulation steps $m$ of MCTS, such that 
\[
\xi_{v}^{(l+1)}\leq\rho\xi_{v}^{(l)},\quad \xi_{p}^{(l+1)}\leq\rho\xi_{v}^{(l)}.
\]
For instance, we can set the depth of MCTS as follows: 
$$H^{(l+1)}=\log_{\gamma}\bigg(\frac{\rho}{|\mA|\max \Big\{c_{v}(n_{l+1}),\frac{2c_{p}(n_{l+1})}{\tau_{l+1}}\Big\}}\bigg)=O\Big(\log \frac{1}{\rho} \Big).$$
As for the number of simulation steps of MCTS, setting\\ $O\big(m_{l+1}^{\eta-1}\big)=|\mA|\gamma^{H^{(l+1)}}\xi_{v}^{(l)}$ is sufficient. That is,
$$m_{l+1}=\kappa_0 \bigg( \frac{\rho^{l+1}} {\max \Big\{c_{v}(n_{l+1}),\frac{2c_{p}(n_{l+1})}{\tau_{l+1}}\Big\}} \bigg)^{\frac{1}{\eta-1}}=O\Big(\rho^{\frac{l+1}{\eta-1}}\Big),$$
where $\kappa_0>0$ is a sufficiently large constant.
At the first iteration, the model is initialized with parameters $\theta_0$ and the leaf node value  in the tree search is set to $V_{\theta_0}$. That is,
$\xi_{v}^{(0)}=C_0$. Therefore, 
\[
\xi_{v}^{(l)}\leq C_0\rho^{l},\quad \xi_{p}^{(l)}\leq C_0\rho^{l}.
\]

\end{proof}

==> ais_tex_files/imple_main_old.tex <==
\section{Implementation: A Concrete Instantiation of the Key Modules}\label{sec:example}



In this section, we demonstrate the applicability of the generic EIS algorithm by giving a concrete instantiation. Specifically, we will use a variant of Monte Carlo Tree Search (MCTS) as the improvement module, the nearest neighbor supervised learning as the supervised learning module and the random sampling policy as the exploration module. Importantly, we show that the technical properties in Section \ref{subsec:properties} are all satisfied. This validates that the properties are not merely technical, but indeed practical, and hence gives a strong support for the generic receipt developed throughout this paper. Due to space limit, we provide high-level discussions here with \emph{informal} technical results. A detailed description with precise statements can be found in Appendix \ref{appendix:example}.

{\bf Improvement Module: MCTS.}
Recall that the improvement module should be capable of providing improved estimates for both the value and policy functions, at the queried state $s$. Since both the value and policy are closely related to the $Q$ function, one simple approach to simultaneously produce improved estimates is to obtain better estimates of $Q^*$ first and then construct the improved estimates of value and policy from $\hat{Q}$. We will take this approach in this example and use MCTS to obtain the $Q$ estimates (see Algorithm \ref{alg:mcts} in Appendix \ref{appendix:example}).   
The following theorem states the property of this specific improvement module, which
%. It is not hard to see that it 
directly implies the desired improvement property, i.e., Property~\ref{property:improvement}.

\begin{thm}[Informal]
Suppose that the state transitions are deterministic. Given the current model $f=(V,\pi)$ such that  
the value model, $V$, satisfies that 
$\E\big[||V- V^*||_\infty\big]\leq \varepsilon_{0,v}.$
Then, with appropriately chosen parameters, for each query state $s_0\in\mathcal{S}$, $ \big(\hat{V}(s_0), \hat{\pi}(\cdot|s_0)\big) = \textrm{Improvement Module}(f,s_0)$, we have: 

\hspace{0.36in}1. $\:$  $
\mathbb{E}\big[\big|\hat{V}(s_0)-V^*(s_0)\big|\big]\leq\zeta_v\cdot\varepsilon_{0,v},\: \textrm{  and  }\: \mathbb{E}\big[D_{\textup{KL}}\big(\hat{\pi}(\cdot|s_0)||P^*_\tau(\cdot|s_0)\big)\big]\leq \zeta_p\cdot\varepsilon_{0,v}.$

 \hspace{0.36in}2. $\:$The above is achieved with a sample complexity of \[O\Big(\big({\tau\cdot\min\{\zeta_v,\zeta_p\}\cdot\varepsilon_{0,v}}\big)^{-2}\cdot \frac{\log({\tau\cdot\min\{\zeta_v,\zeta_p\}})}{\log \gamma}\Big).\]

\end{thm}


 
{\bf Supervised Learning Module: Nearest Neighbor Regression.}
To establish the generalization property, we employ a nearest neighbor supervised learning algorithm for the optimal value function and policy. 
Intuitively, the nearest neighbor approach will generalize if it is always guaranteed to have sufficiently many, say $K$, neighbors in the training data. Informally, consider covering the state space $\mS$ with balls of diameters at most $h$ for some $h>0$. Then, roughly speaking, for generalization, each of the covering balls should have at least $K$ training data. We call the training data \emph{$(h,K)$-representative} if this is the case. Of course, $h$ and $K$ would depend on the temperature $\tau,$ and estimation errors of the training data.  


\begin{prop}[Informal]
Under some regularity conditions,
%on the optimal value function and 
% Suppose Assumption~\ref{assu:smooth} holds. 
 if the training data is representative with respect to appropriate chosen $h>0$ and $K>0$, the nearest neighbor supervised learning satisfies Property~\ref{property:sl}. In particular, given the estimation errors, $\epsilon_v$ and $\epsilon_p$, of the training data, we have 
%  if
% \begin{align}
%     h=\min\Big\{\frac{\varepsilon_v}{L_v},\frac{\sqrt{\varepsilon_p}}{L_p(\tau)}\Big\}, K=\max\Big\{\frac{V_{\max}^{2}}{2\varepsilon_{v}^{2}}\log\Big(\frac{4V_{\max}N_h}{\varepsilon_{v}}\Big),  \frac{1}{\varepsilon_p}\log\Big(\frac{2N_h}{\varepsilon_p}\Big) \Big\}, 
% \end{align}
% we have 
\begin{align*}
\E\left[\left\Vert \vnn-V^{*}\right\Vert _{\infty}\right] & \le 4 \cdot \varepsilon_{v},\\
\E\left[D_{\textup{KL}}\big(\pinn(\cdot|s)\,\Vert\,P^{*}_\tau(\cdot|s)\big)\right] & \le c\cdot\varepsilon_{p},\quad \forall s \in \mS,
\end{align*}
where the constant $c>0$ is independent of $n$, the size of training data. 
\end{prop}

   

{\bf Exploration Module: Random Sampling Policy}
As illustrated in the supervised learning module, the sampled states for nearest neighbor regression should be $(h,K)$-representative. In other words, to satisfy the exploration property, the exploration module must be able to visit a set of $(h,K)$-representative states within a finite expected number of steps. \red{Let $N(h)$ be the }
We show that a uniformly random sampling policy can achieve this.

\begin{prop}[Informal] 
Under some regularity conditions and given the estimation errors, $\epsilon_v$ and $\epsilon_p$, for the value and policy.  Then, the expected number of steps to obtain a set of $(h,K)$-representative states under the random sampling policy is upper bounded by 
$B(\tau,\varepsilon_v,\varepsilon_p)=O\left(\frac{KN(h)}{c_0} \log N(h)\right).$
\end{prop}




{\bf Convergence Guarantees and Sample Complexity of the Instance}
For this instance of the EIS algorithm,
we have shown that each module satisfies the desired properties. Therefore, the convergence result stated in Theorem~\ref{thm:eis_convergence} holds for this specific instance. We now state a more tailored result that takes advantage of the explicit analysis of the instance in this section. In the following, informally, the $c'$s and $V_{\max}$ are some appropriate constants. Please refer to Appendix \ref{appendix:example} for details.




\begin{thm}[Informal]
\label{thm:informal_example_converge}
For a given $\rho\in (0,1)$, there exist appropriately chosen parameters for this instance of Algorithm~\ref{alg:eis} such that:
\begin{enumerate}
\vspace{-0.08in}
    \item The output $f_{L}=(V_L,\pi_L)$ at the end of $L$-th iteration satisfies \begin{align*}
    \E\Big[\big\Vert V_{L} -V^* \big\Vert_\infty \Big] \leq V_{\max}\rho^L \:\textrm{ and }\:
    \E\Big[D_{\text{KL}}\big(\pi_{L}(\cdot|s) \,\Vert\, P_\tau^{*}(\cdot|s)\big)\Big] \leq  \frac{cV_{\max}}{4} \rho^L, \quad \forall s \in \mS.
    \end{align*}
    
  
    \vspace{-0.1in}
    \item \red{With probability at least $1-\delta,$ the above result is achieved with sample complexity of }
    \begin{align*}
        %\sum_{l=1}^{L}M^{(l)}&=
        \sum_{l=1}^{L}c'  \frac{\log(\tau\rho)}{\tau^2\rho^{4l}}\cdot \log \frac{N(c_4 \rho^l)}{\rho}\cdot N(c_4\rho^l) \cdot \log N(c_4\rho^l)\cdot \log\frac{L}{\delta},
     \end{align*}
   
    
    \vspace{-0.1in}
    \item \red{In particular, if $\mS$ is a unit volume hypercube in $\mathbb{R}^d$, then the total sample complexity to achieve $\varepsilon$-error value function and policy is  }
      \begin{align*}
  %\sum_{l=1}^{L}M^{(l)} & =
  O\bigg(  \frac{\log(\tau\rho)}{\tau^2\varepsilon^{d+4}} \cdot \log \big(\frac{1}{\varepsilon}\big)^4 \cdot \log\frac{1}{\delta}\bigg). 
\end{align*} 

\end{enumerate}

\end{thm}

Theorem~\ref{thm:informal_example_converge} states that for a unit volume hypercube, the sample complexity of the instance of EIS algorithm scales as $\widetilde{\Theta}\big(\frac{1}{\varepsilon^{4+d}}\big)$ (omitting the logarithmic factor). Note that the minimax lower bound in Theorem~\ref{thm:lower_bound} 
scale as $\widetilde{\Omega}\big(\frac{1}{\varepsilon^{2+d}}\big)$. Hence, in terms of the dependence on the dimension, the instance we consider here is nearly optimal. 

